Attention Reallocation: Towards Zero-cost and Controllable Hallucination Mitigation of MLLMs

Multi-Modal Large Language Models (MLLMs) stand out in various tasks but still struggle with hallucinations. While recent training-free mitigation methods mostly introduce additional inference overhead via retrospection strategy and contrastive decoding, we propose attention reallocation (AttnReal) to mitigate hallucinations with nearly zero extra cost. Our approach is motivated by the key observations that, MLLM's unreasonable attention distribution causes features to be dominated by historical output tokens, which further contributes to hallucinated responses because of the distribution gap between different token types. Based on the observations, AttnReal recycles excessive attention from output tokens and reallocates it to visual tokens, which reduces MLLM's reliance on language priors and ensures the decoding process depends more on the visual inputs. More interestingly, we find that, by controlling the intensity of AttnReal, we can achieve a wide-range trade-off between the response faithfulness and overall performance. Comprehensive results from different benchmarks validate the effectiveness of AttnReal across six open-source MLLMs and three decoding strategies.

==> tables/CHAIR-main-entire.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{booktabs}
\begin{table*}[htbp]
\caption{CHAIR-half}
\label{tab: chair-half}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Type} &
\multicolumn{3}{c}{LLaVA-1.5} & \multicolumn{3}{c}{LLaVA-1.5-13B} & \multicolumn{3}{c}{MiniGPT-4} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 &  & 
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score \\
\cmidrule(lr){1-11}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 47.0 & 14.3 & 77.1 & 44.8 & 12.8 & 77.9  & 31.0  & 9.6  & 70.6  \\
DoLa             &                                   & 46.8  & 14.3  & 76.9  & -  & -  & -  & 29.2  & 10.1  & 71.5  \\
PAI              &                                   & 29.6  & 7.3  & 76.0  & 35.6  & 9.2  & 77.9  & 24.4  & 9  & 70.9  \\
Ours             &                                   & + & + & + & + & + & + & + & + & + \\
Ours             &                                   & + & + & + & + & + & + & + & + & + \\
\cmidrule(lr){1-11}
Beam Search      & \multirow{6}{*}{Beam Search}      & 51.8  & 15.5  & 77.0  & 49.0  & 13.4  & 78.3  & 34.4  & 10.9  & 70.4  \\
OPERA            &                                   & 48.6  & 14.1  & 76.9  & 40.4  & 12.4  & 76.8  & 28.6  & 10.1  & 69.6  \\
VCD-Beam         &                                   & 52.6  & 16.0  & 74.8  & 48.4  & 14.5  & 75.0  & 32.4  & 9.8  & 69.8  \\
PAI-Beam         &                                   & 35.0  & 10.2  & 75.6  & 40.4  & 12.6  & 77.0  & 24.0  & 8.7  & 69.8  \\
Ours-Beam        &                                   & + & + & + & + & + & + & + & + & + \\
Ours-Beam        &                                   & + & + & + & + & + & + & + & + & + \\
\cmidrule(lr){1-11}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 52.8  & 17.3  & 72.7  & 54.2  & 15.6  & 73.8  & 34.6  & 11.0  & 69.5  \\
VCD              &                                   & 48.4  & 15.1  & 74.3  & 50.0  & 14.5  & 76.0  & 32.0  & 10.3  & 68.8  \\
PAI-Nucleus      &                                   & 39.2  & 10.8  & 74.0  & 41.0  & 12.8  & 76.1  & 23.2  & 9.2  & 70.9  \\
Ours-Nucleus     &                                   & + & + & + & + & + & + & + & + & + \\
Ours-Nucleus     &                                   & + & + & + & + & + & + & + & + & + \\

\bottomrule
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Type} &
\multicolumn{3}{c}{Shikra} & \multicolumn{3}{c}{ mPLUG-Owl2} & \multicolumn{3}{c}{Qwen2-VL} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 &  & 
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score \\
\cmidrule(lr){1-11}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 56.6  & 16.4  & 74.5  & 59.0  & 19.3  & 71.1  & 30  & 8.9  & 77.1  \\
DoLa             &                                   & -  & -  & -  & 58.2  & 18.6  & 71.5  & -  & -  & -  \\
PAI              &                                   & 31  & 8.6  & 74.9  & -  & -  & -  & -  & -  & -  \\
Ours             &                                   & + & + & + & + & + & + & + & + & + \\
Ours             &                                   & + & + & + & + & + & + & + & + & + \\
\cmidrule(lr){1-11}
Beam Search      & \multirow{6}{*}{Beam Search}      & 57.0  & 15.5  & 75.1  & 58.2  & 18.1  & 73.1  & -  & -  & -  \\
OPERA            &                                   & 38.4  & 12.9  & 73.8  & 50.8  & 16.9  & 72.2  & -  & -  & -  \\
VCD-Beam         &                                   & -  & -  & -  & 59.6  & 19.9  & 68.8  & -  & -  & -  \\
PAI-Beam         &                                   & 33.8  & 10.0  & 74.5  & -  & -  & -  & -  & -  & -  \\
Ours-Beam        &                                   & + & + & + & + & + & + & -  & -  & -  \\
Ours-Beam        &                                   & + & + & + & + & + & + & -  & -  & -  \\
\cmidrule(lr){1-11}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 60.8  & 16.1  & 72.5  & 61.2  & 19.8  & 68.9  & -  & -  & -  \\
VCD              &                                   & -  & -  & -  & 58.4  & 20.3  & 68.9  & -  & -  & -  \\
PAI-Nucleus      &                                   & 34.2  & 8.9  & 74.1  & -  & -  & -  & -  & -  & -  \\
Ours-Nucleus     &                                   & + & + & + & + & + & + & -  & -  & -  \\
Ours-Nucleus     &                                   & + & + & + & + & + & + & -  & -  & -  \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/CHAIR-main-part1-v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{booktabs}
\begin{table*}[htbp]
\caption{CHAIR-part1}
\label{tab: chair-part1}
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Type} &
\multicolumn{3}{c}{LLaVA-1.5} & \multicolumn{3}{c}{LLaVA-1.5-13B} & \multicolumn{3}{c}{MiniGPT-4} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 &  & 
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score \\
\cmidrule(lr){1-11}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 47.0 & 14.3 & 77.1 & 44.8 & 12.8 & 77.9  & 31.0  & 9.6  & 70.6  \\
DoLa             &                                   & 46.8  & 14.3  & 76.9  & -  & -  & -  & 29.2  & 10.1  & 71.5  \\
PAI              &                                   & 29.6  & 7.3  & 76.0  & 35.6  & 9.2  & 77.9  & 24.4  & 9.0  & 70.9  \\
\rowcolor{blue!10}\textbf{Ours (CHAIR-aligned)}&              & 30.6 & \textbf{7.0} & \textbf{78.3 \red{($\Uparrow$ 1.2)}} & 36.6 & \textbf{8.7} & \textbf{79.7 \red{($\Uparrow$ 1.8)}} & 25.6 & \textbf{7.7} & 70.9 \\
\rowcolor{green!10}\textbf{Ours (F1-aligned)}            &     & \textbf{23.0 \red{($\Downarrow$ 7.6)}} & \textbf{5.3 \red{($\Downarrow$ 1.7)}} & \textbf{77.3} & \textbf{24.6 \red{($\Downarrow$11.0)}} & \textbf{5.0 \red{($\Downarrow$4.2)}} & \textbf{78.0} & 27.8 & \textbf{8.2 \red{($\Downarrow$0.8)}} & \textbf{71.5} \\
\cmidrule(lr){1-11}
Beam Search      & \multirow{6}{*}{Beam Search}      & 51.8  & 15.5  & 77.0  & 49.0  & 13.4  & 78.3  & 34.4  & 10.9  & 70.4  \\
OPERA            &                                   & 48.6  & 14.1  & 76.9  & 40.4  & 12.4  & 76.8  & 28.6  & 10.1  & 69.6  \\
VCD-Beam         &                                   & 52.6  & 16.0  & 74.8  & 48.4  & 14.5  & 75.0  & 32.4  & 9.8  & 69.8  \\
PAI-Beam         &                                   & 35.0  & 10.2  & 75.6  & 40.4  & 12.6  & 77.0  & 24.0  & 8.7  & 69.8  \\
\rowcolor{blue!10}\textbf{Ours-Beam (CHAIR-aligned)}    &    & 36.6 & \textbf{9.8} & \textbf{78.4 \red{($\Uparrow$ 1.4)}} & \textbf{40.0} & \textbf{9.6} & \textbf{79.5 \red{($\Uparrow$ 1.2)}} & 24.2 &\textbf{6.7} & \textbf{71.4 \red{($\Uparrow$ 1.0)}} \\
\rowcolor{green!10}\textbf{Ours-Beam (F1-aligned)}       &    & \textbf{21.6 \red{($\Downarrow$13.4)}} & \textbf{6.4 \red{($\Downarrow$3.8)}} & \textbf{77.4} & \textbf{27.8 \red{($\Downarrow$12.6)}} & \textbf{6.5 \red{($\Downarrow$6.1)}} & \textbf{78.5} & \textbf{17.2 \red{($\Downarrow$6.8)}} & \textbf{5.5 \red{($\Downarrow$3.2)}} & 70.3 \\
\cmidrule(lr){1-11}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 52.8  & 17.3  & 72.7  & 54.2  & 15.6  & 73.8  & 34.6  & 11.0  & 69.5  \\
VCD              &                                   & 48.4  & 15.1  & 74.3  & 50.0  & 14.5  & 76.0  & 32.0  & 10.3  & 68.8  \\
PAI-Nucleus      &                                   & 39.2  & 10.8  & 74.0  & 41.0  & 12.8  & 76.1  & 23.2  & 9.2  & 70.9  \\
\rowcolor{blue!10}\textbf{Ours-Nucleus (CHAIR-aligned)}    &     & 42.0 & \textbf{10.6} & \textbf{75.0 \red{($\Uparrow$ 0.7)}} & 42.6 & \textbf{10.1} & \textbf{77.6 \red{($\Uparrow$ 1.5)}} & 25.4 & \textbf{7.6} & 70.0 \\
\rowcolor{green!10}\textbf{Ours-Nucleus (F1-aligned)}    &        & 42.2 & \textbf{9.3 \red{($\Downarrow$1.5)}}  & \textbf{74.8} & \textbf{37.2 \red{($\Downarrow$3.8)}} & \textbf{7.9 \red{($\Downarrow$4.9)}} & \textbf{76.2} & 26.0 & 9.9 & 70.5 \\

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/CHAIR-main-part1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{booktabs}
\begin{table*}[htbp]
\caption{CHAIR evaluation results on LLaVA-1.5-7B, LLaVA-1.5-13B and MiniGPT-4. CHAIR$_\text{S}$ and CHAIR$_\text{I}$ (lower is better) reflect the degree of hallucination. F1 score (higher is better) represents for the comprehensive consideration of accuracy and recall.
% CHAIR hallucination evaluation results on three LVLMs. CHAIR [31] is employed as the evaluation metric, where a smaller number indicates less hallucinations. OPERA is a decoding method based on beam search, VCD is a decoding method based on nucleus sampling, and PAI is an inference intervention method that can be collaborated with any decoding method.
}
\label{tab: chair-part1}
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Strategy} &
\multicolumn{3}{c}{LLaVA-1.5-7B~\cite{liu2024visualllava}} & \multicolumn{3}{c}{LLaVA-1.5-13B~\cite{liu2024visualllava}} & \multicolumn{3}{c}{MiniGPT-4~\cite{zhu2023minigpt}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 &  & 
  CHAIR$_\text{S}\downarrow$ &  CHAIR$_\text{I}\downarrow$ &  F1 $\uparrow$ &
  CHAIR$_\text{S}\downarrow$ &  CHAIR$_\text{I}\downarrow$ &  F1 $\uparrow$ &
  CHAIR$_\text{S}\downarrow$ &  CHAIR$_\text{I}\downarrow$ &  F1 $\uparrow$ \\
\cmidrule(lr){1-11}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 47.0 & 14.3 & 77.1 & 44.8 & 12.8 & 77.9  & 31.0  & 9.6  & 70.6  \\
DoLa~\cite{chuang2023dola}             &                                   & 46.8  & 14.3  & 76.9  & -  & -  & -  & 29.2  & 10.1  & 71.5  \\
PAI~\cite{liu2024pai}              &                                   & 29.6  & 7.3  & 76.0  & 35.6  & 9.2  & 77.9  & 24.4  & 9.0  & 70.9  \\
\rowcolor{blue!10}\textbf{Ours (CHAIR-aligned)}&              & \textbf{30.6} & \textbf{7.0} & \textbf{78.3 \small{\red{($\uparrow$1.2)}}} & \textbf{36.6} & \textbf{8.7} & \textbf{79.7 \small{\red{($\uparrow$1.8)}}} & \textbf{25.6} & \textbf{7.7} & \textbf{70.9} \\
\rowcolor{green!10}\textbf{Ours (F1-aligned)}            &     & \textbf{23.0 \small{\red{($\downarrow$6.6)}}} & \textbf{5.3 \small{\red{($\downarrow$1.7)}}} & \textbf{77.3} & \textbf{24.6 \small{\red{($\downarrow$11.0)}}} & \textbf{5.0 \small{\red{($\downarrow$4.2)}}} & \textbf{78.0} & \textbf{27.8} & \textbf{8.2 \small{\red{($\downarrow$0.8)}}} & \textbf{71.5} \\
\cmidrule(lr){1-11}
Beam Search      & \multirow{6}{*}{Beam Search}      & 51.8  & 15.5  & 77.0  & 49.0  & 13.4  & 78.3  & 34.4  & 10.9  & 70.4  \\
OPERA~\cite{huang2024opera}            &                                   & 48.6  & 14.1  & 76.9  & 40.4  & 12.4  & 76.8  & 28.6  & 10.1  & 69.6  \\
VCD-Beam~\cite{leng2024vcd}         &                                   & 52.6  & 16.0  & 74.8  & 48.4  & 14.5  & 75.0  & 32.4  & 9.8  & 69.8  \\
PAI-Beam~\cite{liu2024pai}         &                                   & 35.0  & 10.2  & 75.6  & 40.4  & 12.6  & 77.0  & 24.0  & 8.7  & 69.8  \\
\rowcolor{blue!10}\textbf{Ours-Beam (CHAIR-aligned)}    &    & \textbf{36.6} & \textbf{9.8} & \textbf{78.4 \small{\red{($\uparrow$1.4)}}} & \textbf{40.0} & \textbf{9.6} & \textbf{79.5 \small{\red{($\uparrow$1.2)}}} & \textbf{24.2} &\textbf{6.7} & \textbf{71.4 \small{\red{($\uparrow$1.0)}}} \\
\rowcolor{green!10}\textbf{Ours-Beam (F1-aligned)}       &    & \textbf{21.6 \small{\red{($\downarrow$13.4)}}} & \textbf{6.4 \small{\red{($\downarrow$3.8)}}} & \textbf{77.4} & \textbf{27.8 \small{\red{($\downarrow$12.6)}}} & \textbf{6.5 \small{\red{($\downarrow$6.1)}}} & \textbf{78.5} & \textbf{17.2 \small{\red{($\downarrow$6.8)}}} & \textbf{5.5 \small{\red{($\downarrow$3.2)}}} & \textbf{70.3} \\
\cmidrule(lr){1-11}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 52.8  & 17.3  & 72.7  & 54.2  & 15.6  & 73.8  & 34.6  & 11.0  & 69.5  \\
VCD~\cite{leng2024vcd}              &                                   & 48.4  & 15.1  & 74.3  & 50.0  & 14.5  & 76.0  & 32.0  & 10.3  & 68.8  \\
PAI-Nucleus~\cite{liu2024pai}      &                                   & 39.2  & 10.8  & 74.0  & 41.0  & 12.8  & 76.1  & 23.2  & 9.2  & 70.9  \\
\rowcolor{blue!10}\textbf{Ours-Nucleus (CHAIR-aligned)}    &     & \textbf{42.0} & \textbf{10.6} & \textbf{75.0 \small{\red{($\uparrow$0.7)}}} & \textbf{42.6} & \textbf{10.1} & \textbf{77.6 \small{\red{($\uparrow$1.5)}}} & \textbf{25.4} & \textbf{7.6} & \textbf{70.0} \\
\rowcolor{green!10}\textbf{Ours-Nucleus (F1-aligned)}    &        & \textbf{42.2} & \textbf{9.3 \small{\red{($\downarrow$1.5)}}}  & \textbf{74.8} & \textbf{37.2 \small{\red{($\downarrow$3.8)}}} & \textbf{7.9 \small{\red{($\downarrow$4.9)}}} & \textbf{76.2} & \textbf{26.0} & \textbf{9.9} & \textbf{70.5} \\

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/CHAIR-main-part2-v2.tex <==
\begin{table*}[htbp]
\caption{CHAIR-part2}
\label{tab: chair-part2}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5mm}
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Type} &
\multicolumn{3}{c}{Shikra} & \multicolumn{3}{c}{ mPLUG-Owl2} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 &  & 
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score &
  CHAIR$_\text{S}$ &  CHAIR$_\text{I}$ &  F1 Score \\
\cmidrule(lr){1-8}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 56.6  & 16.4  & 74.5  & 59.0  & 19.3  & 71.1  \\
DoLa             &                                   & -  & -  & -  & 58.2  & 18.6  & 71.5  \\
PAI              &                                   & \underline{31}  & 8.6  & 74.9  & -  & -  & -    \\
\rowcolor{blue!10}\textbf{Ours (CHAIR-aligned)}              &         & 31.2 & \underline{7.6} & \textbf{75.6} & \underline{37.0} & \underline{11.1} & \textbf{75.3} \\
\rowcolor{green!10}\textbf{Ours (F1-aligned)}             &             & \textbf{24.2} & \textbf{5.9} & \underline{75.3} & \textbf{19.8} & \textbf{6.2} & \underline{72.9} \\
\cmidrule(lr){1-8}
Beam Search      & \multirow{6}{*}{Beam Search}      & 57.0  & 15.5  & 75.1  & 58.2  & 18.1  & 73.1    \\
OPERA            &                                   & 38.4  & 12.9  & 73.8  & 50.8  & 16.9  & 72.2    \\
VCD-Beam         &                                   & -  & -  & -  & 59.6  & 19.9  & 68.8   \\
PAI-Beam         &                                   & \underline{33.8}  & 10.0  & 74.5  & -  & -  & -   \\
\rowcolor{blue!10}\textbf{Ours-Beam (CHAIR-aligned)}        &          & 34.2 & \underline{8.1} & \textbf{77.0} & \underline{43.0} & \underline{13.6} & \textbf{75.2}   \\
\rowcolor{green!10}\textbf{Ours-Beam (F1-aligned)}        &             & \textbf{21.8} & \textbf{5.2} & \underline{75.1} & \textbf{22.8} & \textbf{7.9} & \underline{73.2}   \\
\cmidrule(lr){1-8}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 60.8  & 16.1  & 72.5  & 61.2  & 19.8  & 68.9  \\
VCD              &                                   & -  & -  & -  & 58.4  & 20.3  & 68.9   \\
PAI-Nucleus      &                                   & \underline{34.2}  & 8.9  & 74.1  & -  & -  & -  \\
\rowcolor{blue!10}\textbf{Ours-Nucleus (CHAIR-aligned)}      &         & 36.6 & \underline{7.9} & \textbf{76.6} & \underline{36.8} & \underline{11.4} & \textbf{72.3}   \\
\rowcolor{green!10}\textbf{Ours-Nucleus (F1-aligned)}     &             & \textbf{33.0} & \textbf{7.1} & \underline{74.2} & \textbf{28.6} & \textbf{9.0} & \underline{70.4}  \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/CHAIR-main-part2.tex <==
\begin{table*}[htbp]
\caption{CHAIR-part2}
\label{tab: chair-part2}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5mm}
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Decoding Strategy} &
\multicolumn{3}{c}{Shikra~\cite{chen2023shikra}} & \multicolumn{3}{c}{mPLUG-Owl2~\cite{ye2024mplug}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 &  & 
  CHAIR$_\text{S}\downarrow$ &  CHAIR$_\text{I}\downarrow$ &  F1 $\uparrow$ &
  CHAIR$_\text{S}\downarrow$ &  CHAIR$_\text{I}\downarrow$ &  F1 $\uparrow$ \\
\cmidrule(lr){1-8}



Greedy           & \multirow{5}{*}{Greedy Decoding}  & 56.6  & 16.4  & 74.5  & 59.0  & 19.3  & 71.1  \\
DoLa~\cite{chuang2023dola}             &                                   & -  & -  & -  & 58.2  & 18.6  & 71.5  \\
PAI~\cite{liu2024pai}              &                                   & 31  & 8.6  & 74.9  & -  & -  & -    \\
\rowcolor{blue!10}\textbf{Ours (CHAIR-aligned)}              &         & \textbf{31.2} & \textbf{7.6} & \textbf{75.6 \small{\red{($\uparrow$0.7)}}} & \textbf{37.0} & \textbf{11.1} & \textbf{75.3 \small{\red{($\uparrow$3.8)}}} \\
\rowcolor{green!10}\textbf{Ours (F1-aligned)}             &             & \textbf{24.2 \small{\red{($\downarrow$6.8)}}} & \textbf{5.9 \small{\red{($\downarrow$2.7)}}} & \textbf{75.3} & \textbf{19.8 \small{\red{($\downarrow$38.4)}}} & \textbf{6.2 \small{\red{($\downarrow$12.4)}}} & \textbf{72.9} \\
\cmidrule(lr){1-8}
Beam Search      & \multirow{6}{*}{Beam Search}      & 57.0  & 15.5  & 75.1  & 58.2  & 18.1  & 73.1    \\
OPERA~\cite{huang2024opera}            &                                   & 38.4  & 12.9  & 73.8  & 50.8  & 16.9  & 72.2    \\
VCD-Beam~\cite{leng2024vcd}         &                                   & -  & -  & -  & 59.6  & 19.9  & 68.8   \\
PAI-Beam~\cite{liu2024pai}         &                                   & 33.8  & 10.0  & 74.5  & -  & -  & -   \\
\rowcolor{blue!10}\textbf{Ours-Beam (CHAIR-aligned)}        &          & \textbf{34.2} & \textbf{8.1} & \textbf{77.0 \small{\red{($\uparrow$1.9)}}} & \textbf{43.0} & \textbf{13.6} & \textbf{75.2 \small{\red{($\uparrow$2.1)}}}   \\
\rowcolor{green!10}\textbf{Ours-Beam (F1-aligned)}        &             & \textbf{21.8 \small{\red{($\downarrow$12.0)}}} & \textbf{5.2 \small{\red{($\downarrow$4.8)}}} & \textbf{75.1} & \textbf{22.8 \small{\red{($\downarrow$28.0)}}} & \textbf{7.9 \small{\red{($\downarrow$9.0)}}} & \textbf{73.2}   \\
\cmidrule(lr){1-8}
Nucleus Sampling & \multirow{5}{*}{Nucleus Sampling} & 60.8  & 16.1  & 72.5  & 61.2  & 19.8  & 68.9  \\
VCD~\cite{leng2024vcd}               &                                   & -  & -  & -  & 58.4  & 20.3  & 68.9   \\
PAI-Nucleus~\cite{liu2024pai}       &                                   & 34.2  & 8.9  & 74.1  & -  & -  & -  \\
\rowcolor{blue!10}\textbf{Ours-Nucleus (CHAIR-aligned)}      &         & \textbf{36.6} & \textbf{7.9} & \textbf{76.6 \small{\red{($\uparrow$2.5)}}} & \textbf{36.8} & \textbf{11.4} & \textbf{72.3 \small{\red{($\uparrow$3.4)}}}   \\
\rowcolor{green!10}\textbf{Ours-Nucleus (F1-aligned)}     &             & \textbf{33.0 \small{\red{($\downarrow$1.2)}}} & \textbf{7.1 \small{\red{($\downarrow$1.8)}}} & \textbf{74.2} & \textbf{28.6 \small{\red{($\downarrow$29.8)}}} & \textbf{9.0 \small{\red{($\downarrow$11.3)}}} & \textbf{70.4}  \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/Decoding-Overhead-intro.tex <==
\begin{table}[htbp]
\caption{Decoding overhead comparison.}
\label{tab: decoding overhead}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method &
  \begin{tabular}[c]{@{}c@{}}Decoding\\ strategy\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Contrasting \\ decoding\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Candidates \\ per step\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Overhead \\ (GFLOPs) \end{tabular} \\ 
\cmidrule(lr){1-5}
Greedy           & \multirow{4}{*}{Greedy Decoding}  & \ding{55} & 1 & 102.13 / token \\
DoLa             &                          & \ding{51} & 1 & 135.74 / token \\
PAI              &                          & \ding{51} & 1 & 126.56 / token \\
\textbf{Ours}             &                          & \textbf{\ding{55}} & \textbf{1} & \textbf{104.82 / token} \\ 
\cmidrule(lr){1-5}
Beam Search      & \multirow{2}{*}{Beam Search}    & \ding{55} & 5 & 474.76 / token \\
OPERA            &                          & \ding{55} & 5 & 1036.84 / token \\ 
\textbf{Ours-Beam}             &                          & \textbf{\ding{55}} & \textbf{5} & \textbf{483.75 / token} \\ 
\cmidrule(lr){1-5}
Nucleus Sampling & \multirow{2}{*}{Nucleus Sampling} & \ding{55} & 1 & 101.16 / token \\
VCD              &                          & \ding{51} & 1 & 214.65 / token \\ 
\textbf{Ours-Nucleus}             &                          & \textbf{\ding{55}} & \textbf{1} & \textbf{104.82 / token} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/Open-Evaluation-main-part1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
\caption{ GPT-assisted open evaluation.}
\label{tab: open evaluatoin}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Method} &
  \multicolumn{2}{c}{LLaVA-1.5-7B} &
  \multicolumn{2}{c}{LLaVA-1.5-13B} &
  \multicolumn{2}{c}{MiniGPT-4} &
  \multicolumn{2}{c}{Shikra} &
  \multicolumn{2}{c}{mPLUG-Owl2} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
 &
  Correctness &
  Detailedness &
  Correctness &
  Detailedness &
  Correctness &
  Detailedness &
  Correctness &
  Detailedness &
  Correctness &
  Detailedness \\ 
\cmidrule(lr){1-11}
Greedy & 3.22 & 3.35 & 3.38 & 3.43 & 2.8  & 3.25 & 2.99 & 3.23 & 2.66 & \underline{3.1}  \\
DoLa            & 3.25 & \underline{3.41} & - & - & 2.81 & 3.21 & -    & -    & \underline{2.67} & 3.08 \\
OPERA           & \underline{3.31} & \underline{3.41} & 3.36 & 3.37 & 3.03 & 3.22 & 3.02 & 3.14 & 2.65 & 3.07 \\
VCD             & 3.15 & 3.32 & 3.18 & 3.34 & 2.88 & 3.22 & -    & -    & 2.56 & 3    \\
PAI             & 3.24 & 3.29 & \underline{3.4}  & \underline{3.53} & \textbf{3.13} & \textbf{3.36} & \underline{3.13} & \underline{3.28} & -    & -    \\
\textbf{Ours}            & \textbf{3.4}  & \textbf{3.44} & \textbf{3.47} & \textbf{3.55} & \underline{3.07} & \underline{3.35} & \textbf{3.14} & \textbf{3.36} & \textbf{3.04} & \textbf{3.36} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/Open-Evaluation-main-part2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[htbp]
\centering
\caption{ GPT-assisted open evaluation qwen2-vl.}
\label{tab: open evaluatoin qwen}
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{5mm}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Qwen2-VL} \\ 
\cmidrule(lr){2-3} 
                        & Correctness  & Detailedness  \\ 
\cmidrule(lr){1-3}
Greedy                  & 4.08          & 3.93          \\
\textbf{Ours}                    & \textbf{4.17}          & \textbf{3.97}          \\
\bottomrule
\end{tabular}%
}
\end{table}
